Context Attentive Bandits: Contextual Bandit with Restricted Context

We consider a novel formulation of the multi-armed bandit model, which we call the contextual bandit with restricted context, where only a limited number of features can be accessed by the learner at every iteration. This novel formulation is motivated by different online problems arising in clinical trials, recommender systems and attention modeling. Herein, we adapt the standard multi-armed bandit algorithm known as Thompson Sampling to take advantage of our restricted context setting, and propose two novel algorithms, called the Thompson Sampling with Restricted Context(TSRC) and the Windows Thompson Sampling with Restricted Context(WTSRC), for handling stationary and nonstationary environments, respectively. Our empirical results demonstrate advantages of the proposed approaches on several real-life datasets

==> experiments-v1.tex <==
\section{EMPIRICAL EVALUATION}
\label{sec:experimental}
In order to evaluate the proposed approaches for both stationary and nonstationary CBRC problem, we used four datasets from the UCI Machine Learning Repository \footnote{https://archive.ics.uci.edu/ml/datasets.html}. (see  Table \ref{table:Synthetic} for details).

\begin{table}[t]
	\centering
	\caption{Datasets}
	\resizebox{0.99\columnwidth}{!}{
		\begin{tabular}{ l | c | r | r }
			UCI Datasets                  & Instances    & Features   & Classes \\ \hline
			Covertype                & 581 012      & 95           &  7\\
			CNAE-9                   & 1080       & 857          &  9\\
			Internet Advertisements  & 3279         & 1558         &  2\\
			Poker Hand               & 1 025 010    & 11         &  9\\
			
			
		\end{tabular}
	}
	\label{table:Synthetic}
\end{table}

In order to simulate a data stream, we draw samples from the dataset sequentially, starting from the beginning each time we draw the last sample. At each round, the algorithm receives the reward 1 if the instance is classified correctly, and 0 otherwise.  The cumulative regret is computed as the total number of classification mistakes. We compare our algorithms with the following methods:

{\em MAB}: this is the standard TS approach to (non-contextual) MAB setting;

{\em Fullfeatures}: this algorithm uses the CTS with the full set of features;

{\em Random-EI}: this algorithm selects a {\em Random} subset of features of the specified size $d$ at {\em Each Iteration} (thus, {\em Random-EI}), and then invokes the CTS;

{\em Random-fix}: this algorithm invokes CTS on a random subset of $d$ features; however, this subset is selected once prior to seeing any data samples, and remains fixed.

We ran these   algorithms in stationary and non-stationary settings, for different feature subset sizes, such as 5\%, 25\%, 50\% and 75\% of the total number of features. In the figures presented later in this section, we used the parameter, called {\em sparsity}, to denote the percent of features that were {\em not selected}, resulting into the sparsity levels of 95\%, 75\%, 50\% and 25\%, respectively. In the following, we will present our results first for the stationary and then for the non-stationary settings.

\subsection{Stationary case}
\begin{table*}[t]
	\centering
	\caption{Stationary Environment}
	\resizebox{1.54\columnwidth}{!}{
		\begin{tabular}{ l | l | l | l | l | l }
			&  MAB          & Fullfeatures          & TSRC          &   Random-fix   & Random-EI \\ \hline
			Datasets \\ \hline
			Covertype & $70.54\pm 0.30$ &  $ 35.27\pm 0.32$  & $\textbf{53.54}\pm\textbf{1.75}$   & $72.59\pm 2.38$	& $82.69\pm1.87$\\
			CNAE-9 	     &  $79.85 \pm 0.35$    &   $52.01\pm0.20$	  & $\textbf{68.47}\pm \textbf{0.95}$	 & $68.20\pm3.49$	& $80.02\pm 0.23$\\
			Internet Advertisements	      &  $19.22\pm0.20$	                     &   $14.33\pm 0.22$	                & $\textbf{15.21}\pm\textbf{1.20}$	                     & $21.21\pm 1.93$	& $ 23.53\pm\ 1.64$\\
			Poker Hand 	       &  $62.29\pm 0.21$   &   $ 58.57 \pm 0.12$	& $\textbf{58.82}\pm\textbf{0.71}$              & $59.83\pm2.57$   & $58.49\pm0.81$\\
			\hline
		\end{tabular}
	}
	\label{table:AccuSyn}
\end{table*}

\begin{figure*}[h]
	\begin{multicols}{4}
		\includegraphics[height=1in,width=1\linewidth]{5percentstationar.png}\par
		\includegraphics[height=1in,width=1\linewidth]{25percentstationar.png}\par
		\includegraphics[height=1in,width=1\linewidth]{50percentstationar.png}\par
		\includegraphics[height=1in,width=1\linewidth]{75percenstationar.png}\par
	\end{multicols}
\vspace{-0.35in}
	\caption{Stationary Environment (Covertype dataset)}\label{fig:incrst}
\end{figure*}
%\subsubsection{Analysis on all datasets}
Table ~\ref{table:AccuSyn} summarizes our results for the stationary CBRC setting; it represents the average regret, i.e. the misclassification error, computed as the total number of misclassified samples over the number of iterations. This average errors for each algorithm were computed using 10 cyclical iterations over each dataset, and over the four different sparsity levels mentioned above.

As expected, the CTS algorihtm with the full set of features ({\em Fullfeatures}) achieved the the best performance as compared with the rest of the algorithms, underscoring the importance of the amount of context observed in an on-line learning setting. However, when the context is limited, is in CBRC problem considered in this work, our TSRC approach shows superior performance (shown in bold in Table ~\ref{table:AccuSyn}) when compared to the rest of the algorithms, except for the {\em Fullfeatures}, confirming the importance of efficient feature selection in the CBRC setting.
Overall, based on their mean error rate, the top three algorithms were: TSRC (mean error 49.01\%,) Random-fix (mean error 55.46\%) and MAB (mean error 57.98\%), respectively, suggesting that using a fixed randomly selected feature subset may still be a better strategy than not considering any context at all, as in MAB. However,   ignoring the context in MAB may still be a better approach than randomly changing the choice of features at each iteration, as  in {\em Random-EI}, which corresponds to the worst mean error of 61.18\%.

{\bf Sparsity analysis}: Figure \ref{fig:incrst} provides a detailed evaluation of the algorithms for different levels of sparsity, on a Covertype dataset. Ignoring the {\em Fullfeatures} which, as expected, outperforms all methods since it considers the full context, we observe that, in {\bf 95\% sparsity}, {\em TSRC} has the lowest regret out of all methods, followed tightly by {\em MAB}, suggesting that, at a very high sparsity level, ignoring the context ({\em MAB}) is similar to considering only a very small (5\%) fraction of it. In {\bf 75\% sparsity}, we observe that {\em Random-EI} has a lower regret than the {\em Random-fix}.
In {\bf 50\% sparsity}, {\em TSRC} has the lowest regret, followed closely by the {\em Random-fix}, which implies that, at some levels of sparsity, random subset selection can perform almost as good as our optimization strategy. Again, we observe that {\em Random-fix} performs better that the {\em Randon-EI}, where the performance of the latter is close to the MAB without any context. In {\bf 25\% sparsity}, we observe that TSRC perform as good as {\em Fullfeatures}, which implies that at this sparsity level, our approach was able to select the optimal feature subset.

\subsection{Non-stationary Case}
In this setting, for each dataset, we run the experiments for $3 * 10^6$ iterations, where we change the label of class at each  $5*10^5$ iteration to simulate the non-stationarity. We evaluate our {\em WTSRC} algorithm for the nonstationary CBRC problem against our stationary-setting TSRC method, and against the same five baseline methods we presented before. The Table ~\ref{table:AccuSyn1} reports the mean error (regret) over all iterations and over the same for level of sparsity as before. Overall, we observed that the {\em WTSRC} performs the best, confirming the effectiveness of using our time-windows approach in a non-stationary on-line learning setting.
Our top three performing algorithms were {\em WTSRC}, {\em Fullfeatures} and {\em TSRC}, in that order, which underscores the importance of the size of the observed context even in the non-stationary setting.

\begin{table*}[ht]
	\centering
	\caption{Non-Stationary Environment}
	\resizebox{1.69\columnwidth}{!}{
		\begin{tabular}{ l | l | l | l | l | l | l }
			&  MAB          & Fullfeatures          & TSRC          &   Random-fix   & Random-EI  & WTSRC\\ \hline
			Datasets \\ \hline
			Covertype  &$69.72\pm 4.30$ &   $ 68.54\pm 2.10$  & $76.12\pm2.86$   & $80.96\pm2.19$	& $ 80.71\pm2.22 $ 	& $\textbf{60.56 }\pm\textbf{2.95}$ \\
			CNAE-9 	 &  $ 74.34 \pm 5.39 $   &  $ 69.21\pm 2.12 $	  & $ 71.87\pm 4.5$	 & $ 79.87 \pm 4.5 $	& $76.21 \pm 1.90$ & $\textbf{65.56 }\pm\textbf{1.05}$  \\
			Internet Advertisements &  $43.99 \pm 3.85$  &  $ 40.21\pm 1.87 $ & $42.01 \pm 1.79 $ & $40.04 \pm4.52 $	& $40.56\pm1.19$ 	& $\textbf{38.06 }\pm\textbf{0.85}$\\
			Poker Hand 	            &  $82.90\pm4.03$ &   $82.44\pm0.43$	 & $78.86 \pm 1.25$ & $79.99 \pm 1.48$ & $79.81 \pm0.48$ 	& $\textbf{77.56 }\pm\textbf{1.79}$ \\
			\hline
		\end{tabular}
	}
	\label{table:AccuSyn1}
\end{table*}

\begin{figure*}[h]
	\begin{multicols}{4}
		\includegraphics[height=1in,width=1\linewidth]{5percentstationarnt.png}\par
		\includegraphics[height=1in,width=1\linewidth]{25percentstationarnt.png}\par
		\includegraphics[height=1in,width=1\linewidth]{50percentstationarnt.png}\par
		\includegraphics[height=1in,width=1\linewidth]{75percentstationarnt.png}\par
	\end{multicols}
\vspace{-0.35in}
	\caption{Non-Stationary Environment (Covertype dataset)}\label{fig:incr}
\end{figure*}
{\bf Sparsity analysis}: Figure \ref{fig:incr} provides a more detailed evaluation of the algorithms for different levels of sparsity, on a covtype dataset. The {\em Fullfeatures}, as expected, has the same performance on different level of sparsity, since it has the access to all features. We observe that in {\bf95 \% sparsity}, {\em MAB} has the lowest regret, as compared with the {\em Random-EI} and {\em Random-fix}, which implies that, at high sparsity levels, ignoring the context can be better then even considering a small random subset of it. In {\bf75 \% sparsity}, {\em TSRC} yields the best result, implying that even in a non-stationary environment, a stationary strategy for best subset selection can be beneficial. In {\bf50 \% sparsity}, both {\em Random-Fix} and {\em Randon-EI} yield the worst results, implying that random selection is not a good strategy at this sparsity level in non-stationary environment. {\bf25 \% sparsity}, {\em WTSRC}, outperforms all other algorithms, demonstrating the advantages of a dynamic feature-selection strategy in a non-stationary setting.





==> experiments_v0.tex <==
\section{EMPIRICAL EVALUATION}
\label{sec:experimental}
In order to evaluate the proposed approaches for both stationary and nonstationary CBRC problem, we used four datasets from the UCI Machine Learning Repository \footnote{https://archive.ics.uci.edu/ml/datasets.html}, Covertype, CNAE-9, Internet Advertisements and Poker Hand.
In order to simulate a data stream, we draw samples from the dataset sequentially, starting from the beginning each time we draw the last sample. At each round, the algorithm receives the reward 1 if the instance is classified correctly, and 0 otherwise. The cumulative regret is computed as the total number of classification mistakes.

We compare our algorithms with the following competing methods: 
\begin{itemize}
\item {\em MAB}: this is the standard Thomspon Sampling approach to (non-contextual) multi-arm bandit setting.
\item {\em Fullfeatures}: this algorithm uses the CTS with the full set of features.
\item {\em Random-EI}: this algorithm selects a {\em Random} subset of features of the specified size $d$ at {\em Each Iteration} (thus, {\em Random-EI}), and then invokes the CTS.
\item{\em Random-fix}: similarly to {\em Random-EI}, this algorithm invokes CTS on a random subset of $d$ features; however, this subset is selected once prior to seeing any data samples, and remains fixed.
\end{itemize}


We ran the above algorithms and our proposed TSRC and WTSRC methods, in stationary and non-stationary settings, respectively, for different feature subset sizes, such as 5\%, 25\%, 50\% and 75\% of the total number of features. In the Figures presented later in this section, we used the parameter, called {\em sparsity}, to denote the percent of features that were {\em not selected}, resulting into the sparsity levels of 95\%, 75\%, 50\% and 25\%, respectively.  In the following sections, we will present our results first for the stationary and then for the non-stationary settings.


\subsection{Stationary case}
%\subsubsection{Analysis on all datasets}
Table ~\ref{table:AccuSyn} summarizes our results for the stationary CBRC setting; it represents the average regret, i.e. the misclassification error, computed as the total number of misclassified samples over the number of iterations. This average errors for each algorithm were computed using 10 cyclical iterations over each dataset, and over the four different sparsity levels mentioned above.

As expected, the CTS algorihtm with the full set of features ({\em Fullfeatures}) achieved the the best performance as compared with the rest of the algorithms, underscoring the importance of the amount of context observed in an on-line learning setting.
However, when the context is limited, is in CBRC problem considered in this work, our TSRC approach shows superior performance (shown in bold in Table ~\ref{table:AccuSyn}) when compared to the rest of the algorithms, except for the {\em Fullfeatures}, confirming the importance of efficient feature selection in the CBRC setting.
Over, based on their mean error rate, the top three algorithms were TSRC (mean error 49.01\%) Random-fix (mean error 55.46\%) and MAB (mean error 57.98\%), respectively, suggesting that using a fixed randomly selected feature subset may still be a better strategy than not considering any context, as in MAB. However, as it turns out, ignoring the context in MAB may still be a better approach than randomly changing the choice of feature at each iteration in {\em Random-EI} which results into the worst mean error of 61.18\%.

\begin{table*}[ht]
	\centering
	\caption{Stationary Environment}
	\resizebox{1.54\columnwidth}{!}{
		\begin{tabular}{ l | l | l | l | l | l }
			&  MAB          & Fullfeatures          & TSRC          &   Random-fix   & Random-EI \\ \hline
			Datasets \\ \hline
			Covertype & $70.54\pm 0.30$ &  $ 35.27\pm 0.32$  & $\textbf{53.54}\pm\textbf{1.75}$   & $72.59\pm 2.38$	& $82.69\pm1.87$\\
			CNAE-9 	     &  $79.85 \pm 0.35$    &   $52.01\pm0.20$	  & $\textbf{68.47}\pm \textbf{0.95}$	 & $68.20\pm3.49$	& $80.02\pm 0.23$\\
			Internet Advertisements	      &  $19.22\pm0.20$	                     &   $14.33\pm 0.22$	                & $\textbf{15.21}\pm\textbf{1.20}$	                     & $21.21\pm 1.93$	& $ 23.53\pm\ 1.64$\\
			Poker Hand 	       &  $62.29\pm 0.21$   &   $ 58.57 \pm 0.12$	& $\textbf{58.82}\pm\textbf{0.71}$              & $59.83\pm2.57$   & $58.49\pm0.81$\\
			\hline
		\end{tabular}
	}
	\label{table:AccuSyn}
\end{table*}

\subsection{Non-stationary Case}
In this setting, for each dataset, we run the experiments for $3 * 10^6$ iterations, where we change the label of class at each $5*10^5$ iteration to simulate the non-stationarity. We evaluate our {\em WTSRC} algorithm for the non-stationary CBRC problem against our stationary-setting TSRC method, and against the same five baseline methods we presented before.
Similarly to the stationary case evaluation, the Table ~\ref{table:AccuSyn1} reports the mean error (regret) over all iterations and over the same for level of sparsity as before. Overall, we observed that the {\em WTSRC} performs the best, confirming the effectiveness of using our time-windows approach in a non-stationary on-line learning setting.
Our top three performing algorithms were {\em WTSRC}, {\em Fullfeatures} and {\em TSRC}, in that order, which underscores the importance of the size of the observed context even in the non-stationary on-line learning setting.

\begin{table*}[ht]
	\centering
	\caption{Non-Stationary Environment}
	\resizebox{1.69\columnwidth}{!}{
		\begin{tabular}{ l | l | l | l | l | l | l }
			&  MAB          & Fullfeatures          & TSRC          &   Random-fix   & Random-EI  & WTSRC\\ \hline
			Datasets \\ \hline
			Covertype  &$69.72\pm 4.30$ &   $ 68.54\pm 2.10$  & $76.12\pm2.86$   & $80.96\pm2.19$	& $ 80.71\pm2.22 $ 	& $\textbf{60.56 }\pm\textbf{2.95}$ \\
			CNAE-9 	 &  $ 74.34 \pm 5.39 $   &  $ 69.21\pm 2.12 $	  & $ 71.87\pm 4.5$	 & $ 79.87 \pm 4.5 $	& $76.21 \pm 1.90$ & $\textbf{65.56 }\pm\textbf{1.05}$  \\
			Internet Advertisements &  $43.99 \pm 3.85$  &  $ 40.21\pm 1.87 $ & $42.01 \pm 1.79 $ & $40.04 \pm4.52 $	& $40.56\pm1.19$ 	& $\textbf{38.06 }\pm\textbf{0.85}$\\
			Poker Hand 	            &  $82.90\pm4.03$ &   $82.44\pm0.43$	 & $78.86 \pm 1.25$ & $79.99 \pm 1.48$ & $79.81 \pm0.48$ 	& $\textbf{77.56 }\pm\textbf{1.79}$ \\
			\hline
		\end{tabular}
	}
	\label{table:AccuSyn1}
\end{table*}

==> lowerbound-nonstat.tex <==
We will now derive the lower bound on the expected regret in non-stationary CBRC setting with the above assumptions, for any algorithm solving this problem. The only assumption about the algorithm is that it knows about the fixed-size stationarity windows, but not their actual, size and uses $w$ as an approximation of $v$.
{\small\begin{thm}\label{theorem3}
	Let $v$ be the stationary window size, and let $w$ is the stationary window size set by an algorithm for solving the CBRC problem in a non-stationary environment. Then the accumulated expected regret $R$ is lower-bounded by
	\begin{eqnarray*}
		E[R(T)]> \lfloor T/v \rfloor [\gamma \sqrt{\tau d}+\gamma' \sqrt{(w-\tau)d}],
	\end{eqnarray*}
	with $E(\tau) > m \sqrt{Kw}$.
\end{thm}}
\begin{proof}
	Let us assume that the algorithm's estimate $w$ of the stationary window size is exact, i.e. $w=v$; otherwise, the expected regret would only increase. We can decompose the time window $T$ into ${\lfloor T/v \rfloor }$ stationary intervals, each of length $v=w$, and the remaining interval of length $0 \leq w' < w$. Then the expected regret over $T$ can be lower-bounded by the sum of expected regrets $E(R_s(w))$ for stationary CBRC problem on each stationary window; since there are $\lfloor T/v \rfloor$ such windows, we get
	{\small\begin{eqnarray*}
		E(R(T)) \geq \lfloor T/v \rfloor E(R_s(w)).
	\end{eqnarray*}}
	Combining this bound with the following result of the Theorem \ref{theorem1}
	{\small\begin{eqnarray*}
		E(R_s(w))>\gamma \sqrt{\tau d}+\gamma' \sqrt{(w-\tau)d},
	\end{eqnarray*}}
	where $E(\tau) > m \sqrt{KT}$, concludes the proof.
\end{proof}


==> lowerbound-stat.tex <==
However, before introducing an algorithm for solving the above CBRC problem, we will derive a lower bound on the expected regret of any algorithm used to solve this problem. We will now state some lemmas used later in our proof; just to refresh our memory regarding the notation used, $T$ is the number of iterations, $N$ is the total number of features (context size), and $d \leq N$ is the feature subset (restricted context) size.

{\small\begin{ex}\label{fact:lowCB} \cite{ChuLRS11}
For any algorithm solving the {\em contextual bandit} problem with the context size $d$, there exists a constant $\gamma > 0$ such that the lower bound of the expected regret accumulated by the algorithm over $T$ iterations is lower-bounded as follows:
\begin{eqnarray*}
E[R(T)]>\gamma \sqrt{Td}.
\end{eqnarray*}
\end{ex}}
%{\bf TODO: We need to check that we can actually apply this bound to our setting given the differences highlighted earlier.}

We will use combinatorial bandit setting to select feature subsets;
here $N$ corresponds to the number of combinatorial bandit's arms and $d$ corresponds to the size of arm subset.
	


{\small\begin{ex}\label{fact:lowComB} \cite{combes2015combinatorial}
The lower bound of the expected regret for any algorithm in the {\em combinatorial bandit} problem with $K$ arms, where $K > 2m$ and $m$ is the size of the selected arm subset, is given by:
\begin{eqnarray*}
E[R(T)]>m \sqrt{KT}.
\end{eqnarray*}
\end{ex}}
In our feature-selection combinatorial bandit setting, in the above lemma, $K = N$ and $m=d$.
We will now derive the lower bound on the expected regret of any algorithm solving our CBRC problem.



{\small\begin{thm}\label{theorem1}
Let $\pi(\mathbf{c}^d) \in \Pi^d$ denote a policy computed by a particular algorithm for solving CBRC problem, on a feature subset of size $d$. % We will assume that there exists an {\em optimal} subset of features $M^*$ of size $d \leq D$ such that $E(R(\pi^{d},T)) = E(R(\pi^{D},T))$, where an extended notation $R(\pi^{d},T)$ specifies the regret for the hypothesis computed over a subset of features of size $d$.
Then there exist constants $\gamma > 0$ and $\gamma' > 0$ such that the lower bound of the expected regret accumulated by the algorithm over $T$ iterations is lower-bounded as follows:
\begin{eqnarray*}
E[R(T)]>\gamma \sqrt{\tau_1 d}+\gamma' \sqrt{(T-\tau_1) d},
\end{eqnarray*}
\end{thm}}
where $E(\tau_1) > d \sqrt{NT}$.

\begin{proof}
In CBRC setting, the reward received at time $t$ depends both on the choice of the feature subset (restricted context), and on the choice of an arm based on this subset.
%Let $M^*$ be an optimal subset of $d$ features, i.e. the one producing minimal regret over all subsets of given size, assuming an optimal arm-selection policy for any fixed subset of features.

We will now split the set of time points, as well as the regret, in two parts, i.e. $T=\tau_1+\tau_2$ and
{\small\begin{eqnarray*}
R(T)=R(\tau_1)+R(\tau_2 ),
\end{eqnarray*}}
where $\tau_1$ is the number of time points within the initial $T$ iterations at which a sub-optimal subset of the features was selected. Then $R(\tau_2 )$ is the regret of a contextual bandit over optimal subset, with the lower bound on its expected values given by Lemma 1, and $R(\tau_1)$ is the regret accumulated over various suboptimal subsets at different time points in $\tau_1$, and thus its expected value is {\em lower-bounded} by the contextual bandit's regret on a fixed subset, i.e.
%(we denote this set of time points as $T_1$, $|T_1|=\tau_1$),
%and $\tau_2 $ is the rnumber of time points when the optimal subset $M^*$
%(or, more generally any other optimal subset in case there are multiple subsets satisfying $E(R(\pi^{d},T)) = E(R(\pi^{D},T))$ of the features was used; we denote the latter set of time points as $T_2$, $|T_2|=\tau_2$.
%Recall that $\pi(\mathbf{c}^d)$ denotes a hypothesis computed by a given algorithm on a feature subset of size $d$. Then the regret could be expressed as
%\begin{eqnarray*}
%R(T)=R(\sum_{t \in T_1} \pi^{d}(c))+R(\sum_{t \in T_2}\pi^{d}(c))
%\end{eqnarray*}
%Since, by the assumption above, for the optimal subset $M^*$ we have $E(R(\pi^{d},T)) = E(R(\pi^{D},T))$, we obtain
%\begin{eqnarray*}
%R(T)=R(\sum_{\tau_1} \pi(\mathbf{c}^d))+R(\sum_{\tau_2}\pi(\mathbf{c}^d)),
%\end{eqnarray*}
%and thus, for the expected regret,
{\small\begin{eqnarray*}
E[R(T)] \geq E[R(\tau_1)]+E[R(\tau_2 )],
\end{eqnarray*}}
and, using Lemma \ref{fact:lowCB} we get
{\small\begin{eqnarray*}
E[R(T)]>\gamma \sqrt{ \tau_1 d}+\gamma' \sqrt{\tau_2 d},
\end{eqnarray*}}
which gives us the main result of this lemma, once we substitute $\tau_2= T-\tau_1$.
Furthermore, $\tau_1$ is exactly the {\em combinatorial} bandit regret since, by definition, it denotes the number of time points within the first $T$ iterations at which a sub-optimal subset of the features was selected; thus, according to Lemma \ref{fact:lowComB}, $\tau_1 > d \sqrt{NT}$, which concludes the proof.
\end{proof}

==> problem_v0.tex <==
% TO DO
% 1. explain relation between our contextual and Schapire's contextual bandit


\section{PROBLEM SETTING}
\label{sec:statement}
In this section, we define a new type of a bandit problem, the {\em contextual bandit with restricted context (CBRC)}, present two algorithms for solving this problem, in stationary and in non-stationary settings, respectively, and derive
 theoretical results on regret bounds in both settings. In order to address the combinatorial task of feature subset (i.e., restricted context) selection we will build upon the {\em combinatorial bandit} setting \cite{durand2014thompson}, and employ {\em Thompson Sampling (TS)} approach \cite{AgrawalG12}.
 %For definitions and background on contextual and combinatorial bandits, as well as TS algorithm, see the Appendix.

\subsection{Contextual Bandit with Restricted Context in Stationary Environment (CBRC)}


We will now introduce a novel setting: contextual bandit with {\em restricted context}, where the agent cannot observe the full context at any round; instead, it can only request a bounded-size subset of the context and use it to select an action. The objective is to identify a feature subset resulting into maximal cumulative reward. %Below we give a formal definition of the problem.

Let $\textbf{c}^d(t)\in \mathbf{R}^d$ denote a value assignment to a subset of features $ C^d \subseteq C$, $|C^d|=d$, where $d \leq N$ is an upper bound on the feature subset size, and let $k(t)=\pi(\textbf{c}^d(t))$ be an arm selected at time $t$ according to the policy $\pi$. The sequence $((\textbf{c}(1),$ $\textbf{r}(1)),...,(\textbf{c}(t)$, $\textbf{r}(T)))$ represents the history of contexts and rewards obtained at each iteration up to the time point $T$, and is a realization of some stochastic process. Algorithm \ref{alg:CBP} below summarizes the problem setting for the {\em CBRC}.

\begin{small}
\begin{algorithm}[H]
	\caption{ The CBRC Problem Setting}
	% \label{alg.2}
	\label{alg:CBP}
	\begin{algorithmic}[1]
		\STATE {\bfseries }\textbf{Repeat}
		\STATE {\bfseries } $(c(t),r(t))$ is drawn according to $D_{c,r}$
		\STATE {\bfseries } The player chooses a subset $C^d \subseteq C, |C^d|=d$ 
\STATE{\bfseries} The values of $\textbf{c}^d(t)$ of features in $C^d$ are revealed
\STATE{\bfseries} The player chooses an arm $k(t) = \pi(\mathbf{c}^d(t))$
				\STATE {\bfseries } The reward $r_{k(t)}$ is revealed
		\STATE {\bfseries } The player updates its policy $\pi$
			\STATE {\bfseries } $t=t+1$
		\STATE {\bfseries }\textbf{Until} t=T
	\end{algorithmic}
\end{algorithm}
\end{small}



{\small\begin{definition}[Cumulative regret]
Let $\Pi^d = \{\pi(\mathbf{c}^d): \mathbf{R}^d \rightarrow A\}$, where $\mathbf{c}^d$ is an assignment to features in $C^d \subseteq C$, $\forall C^d$ such that $ |C^d| = d$,
i.e. the set of all possible policies $\pi(\textbf{c}^d)$ restricted to some context subset of size $d$, where $\textbf{c}^d$ denotes a
particular sample in the feature subspace defined by feature $C^d$.
%and let $\pi^d_t(\textbf{c}^d) \in \Pi^d$ be a policy computed by the CBRC-solving algorithm at the iteration $t$, under the constraint $d$ on the size of the restricted context; this policy can be also viewed as a compound functions $\pi^d_t(\textbf{c}^d)= f(\textbf{c}^d(\textbf{c}))$, which includes the choice of the restricted context $\textbf{c}^d$, given the full context $\textbf{c}$, followed by the choice of the action in $A$ as prescribed by the function $f(x)$.
 Then the regret of a CBRC-solving algorithm accumulated during $T$ iterations is given as:
\begin{equation*}
R(T) = \max_{\pi \in \Pi^d } \sum ^{T}_{t=1} r_{\pi(\textbf{c}^d(t))}(t) - \sum^{T}_{t=1} r_{k(t)}(t).
\end{equation*}
\end{definition}}
%{\bf TODO: Note the difference in reward definition as compared to Chu's paper; will this affect applicability of their regret bounds to our case?}

The objective of a contextual bandit algorithm, which learns the hypothesis $\pi(T)$ over $T$ iterations, is to minimize the cumulative regret $R(T)$. In the future, we will often denote it simply as $R(T)$ when it is clear from the context which hypothesis $\pi$ is used (e.g., for a specific algorithm). However, before introducing an algorithm for solving the above CBRC problem, we will derive a lower bound on the expected regret of any algorithm used to solve this problem. We will now state some lemmas used later in our proof; just to refresh our memory regarding the notation used, $T$ is the number of iterations, $N$ is the total number of features (context size), and $d \leq N$ is the feature subset (restricted context) size.

{\small\begin{ex}\label{fact:lowCB} \cite{ChuLRS11}
For any algorithm solving the {\em contextual bandit} problem with the context size $d$, there exists a constant $\gamma > 0$ such that the lower bound of the expected regret accumulated by the algorithm over $T$ iterations is lower-bounded as follows:
\begin{eqnarray*}
E[R(T)]>\gamma \sqrt{Td}.
\end{eqnarray*}
\end{ex}}
%{\bf TODO: We need to check that we can actually apply this bound to our setting given the differences highlighted earlier.}

We will use combinatorial bandit setting to select feature subsets;
here $N$ corresponds to the number of combinatorial bandit's arms and $d$ corresponds to the size of arm subset.
	


{\small\begin{ex}\label{fact:lowComB} \cite{combes2015combinatorial}
The lower bound of the expected regret for any algorithm in the {\em combinatorial bandit} problem with $K$ arms, where $K > 2m$ and $m$ is the size of the selected arm subset, is given by:
\begin{eqnarray*}
E[R(T)]>m \sqrt{KT}.
\end{eqnarray*}
\end{ex}}
In our feature-selection combinatorial bandit setting, in the above lemma, $K = N$ and $m=d$.
We will now derive the lower bound on the expected regret of any algorithm solving our CBRC problem.



{\small\begin{thm}\label{theorem1}
Let $\pi(\mathbf{c}^d) \in \Pi^d$ denote a policy computed by a particular algorithm for solving CBRC problem, on a feature subset of size $d$. % We will assume that there exists an {\em optimal} subset of features $M^*$ of size $d \leq D$ such that $E(R(\pi^{d},T)) = E(R(\pi^{D},T))$, where an extended notation $R(\pi^{d},T)$ specifies the regret for the hypothesis computed over a subset of features of size $d$.
Then there exist constants $\gamma > 0$ and $\gamma' > 0$ such that the lower bound of the expected regret accumulated by the algorithm over $T$ iterations is lower-bounded as follows:
\begin{eqnarray*}
E[R(T)]>\gamma \sqrt{\tau_1 d}+\gamma' \sqrt{(T-\tau_1) d},
\end{eqnarray*}
\end{thm}}
where $E(\tau_1) > d \sqrt{NT}$.

\begin{proof}
In CBRC setting, the reward received at time $t$ depends both on the choice of the feature subset (restricted context), and on the choice of an arm based on this subset.
%Let $M^*$ be an optimal subset of $d$ features, i.e. the one producing minimal regret over all subsets of given size, assuming an optimal arm-selection policy for any fixed subset of features.

We will now split the set of time points, as well as the regret, in two parts, i.e. $T=\tau_1+\tau_2$ and
{\small\begin{eqnarray*}
R(T)=R(\tau_1)+R(\tau_2 ),
\end{eqnarray*}}
where $\tau_1$ is the number of time points within the initial $T$ iterations at which a sub-optimal subset of the features was selected. Then $R(\tau_2 )$ is the regret of a contextual bandit over optimal subset, with the lower bound on its expected values given by Lemma 1, and $R(\tau_1)$ is the regret accumulated over various suboptimal subsets at different time points in $\tau_1$, and thus its expected value is {\em lower-bounded} by the contextual bandit's regret on a fixed subset, i.e.
%(we denote this set of time points as $T_1$, $|T_1|=\tau_1$),
%and $\tau_2 $ is the rnumber of time points when the optimal subset $M^*$
%(or, more generally any other optimal subset in case there are multiple subsets satisfying $E(R(\pi^{d},T)) = E(R(\pi^{D},T))$ of the features was used; we denote the latter set of time points as $T_2$, $|T_2|=\tau_2$.
%Recall that $\pi(\mathbf{c}^d)$ denotes a hypothesis computed by a given algorithm on a feature subset of size $d$. Then the regret could be expressed as
%\begin{eqnarray*}
%R(T)=R(\sum_{t \in T_1} \pi^{d}(c))+R(\sum_{t \in T_2}\pi^{d}(c))
%\end{eqnarray*}
%Since, by the assumption above, for the optimal subset $M^*$ we have $E(R(\pi^{d},T)) = E(R(\pi^{D},T))$, we obtain
%\begin{eqnarray*}
%R(T)=R(\sum_{\tau_1} \pi(\mathbf{c}^d))+R(\sum_{\tau_2}\pi(\mathbf{c}^d)),
%\end{eqnarray*}
%and thus, for the expected regret,
{\small\begin{eqnarray*}
E[R(T)] \geq E[R(\tau_1)]+E[R(\tau_2 )],
\end{eqnarray*}}
and, using Lemma \ref{fact:lowCB} we get
{\small\begin{eqnarray*}
E[R(T)]>\gamma \sqrt{ \tau_1 d}+\gamma' \sqrt{\tau_2 d},
\end{eqnarray*}}
which gives us the main result of this lemma, once we substitute $\tau_2= T-\tau_1$.
Furthermore, $\tau_1$ is exactly the {\em combinatorial} bandit regret since, by definition, it denotes the number of time points within the first $T$ iterations at which a sub-optimal subset of the features was selected; thus, according to Lemma \ref{fact:lowComB}, $\tau_1 > d \sqrt{NT}$, which concludes the proof.
\end{proof}

\subsubsection{Thompson Sampling with Restricted Context}
\label{subsec:UCB}
We propose here an algorithm solve the stationary CBRC problem, called {\em Thompson Sampling with Restricted Context (TSRC)}, and is summarized in the algorithm \ref{alg:TSRC}. In TSRC, the combinatorial task of selecting the best subset of features is treated as a combinatorial bandit problem, and the decision-making part as a CMAB problem, respectively.
Let $n_i(t)$ be the number of times the $i$-th feature has been selected so far, let be $r^f_i(t)$ the cumulative reward associated with the feature $i$, and let $r_k(t)$ be the reward associated with choosing the arm $k$ at time $t$. The algorithm takes as an input the desired number of features $d$, as well as the initial values of the Beta distribution parameters.
At each iteration $t$, we update the values of those parameters, $S_i$ and $F_i$ (steps 5 and 6), to represent the current total number of successes and failures, respectively, and then sample the ''probability of success'' parameter $\theta_i$ 
from the corresponding $Beta$ distribution, separately for each feature $i$ (step 7). 
We select the best subset of features, $C^d \subseteq C, |C^d|=d$, which maximizes the sum of those parameters (step 9); note that implementing this step does not actually require combinatorial search\footnote{Since the individual rewards $\theta_i$ are non-negative (recall that they follow Beta-distribution), we can simply select the set $C^d$ of $d$ arms with the highest
individual rewards $\theta_i(t)$.}
Once a subset of features is selected using the combinatorial bandit approach, we switch to the contextual bandit setting % part %(Algorithm 3) 
in steps 10-13, to choose an arm based on the context consisting now of a subset of features. Finally, the reward $r_k(t)$ for choosing an arm $k$ is observed, and relevant parameters are updated.

\begin{small}
\begin{algorithm}[h]
 \caption{Thompson Sampling with Restricted Context}
% \label{alg.2}
\label{alg:TSRC}
\begin{algorithmic}[1]
 \STATE {\bfseries }\textbf{Require:} The size $d$, the initial values $S_i(0)$ and $F_i(0)$ of the Beta distribution parameters. $C^d$ denotes an arbitrary subset of $C$ of size $d$.

 \STATE {\bfseries }\textbf{Initialize:} $\forall k \in \{1,...,K\}, B_k=I_d$,
 $\hat{\mu_k}= 0_d, g_k = 0_d$, and $\forall i \in \{1,...,N\}$, $n_i(0)=0$, $r^f_i(0)=0$.

 \STATE {\bfseries }\textbf{Foreach} $t = 1, 2, . . . ,T$ \textbf{do}

 \STATE {\bfseries }\quad\textbf{Foreach} context feature $i= 1,...,N$ \textbf{do}
 \STATE {\bfseries }\quad\quad $S_i(t)=S_i(0)+r_i(t-1)$
 \STATE {\bfseries } \quad\quad$F_i(t)=F_i(0)+n_i(t-1)-r_i(t-1)$
 \STATE {\bfseries } \quad\quad Sample $\theta_i$ from $ Beta(S_i(t), F_i(t))$ distribution 
\STATE {\bfseries } \quad\textbf{End do}
 \STATE {\bfseries }\quad Select $C^d(t)= argmax_{C^d \subseteq C, |C^d|=d} \sum_{i \in C^d } \theta_i$
 \STATE {\bfseries }\quad\textbf{Foreach} arm $k= 1,...,K$ \textbf{do}
 \STATE {\bfseries }\quad \quad Sample $\tilde{\mu_k}$ from $N(\hat{\mu_k}, v^2 B_k^{-1})$ distribution.
 \STATE {\bfseries } \quad\textbf{End do}
 \STATE {\bfseries }\quad Select arm $k(t)= \underset{k\subset \{1,...,K\} }{argmax} \ C^d(t)^\top \tilde{\mu_k} $
 \STATE {\bfseries }\quad Observe $r_{k}(t)$
\STATE {\bfseries }\quad\textbf{if} $r_{k}(t)=1$ \textbf{then}
\STATE \quad\quad$B_k= B_{k}+ \textbf{c}^d(t)\textbf{c}^d(t)^{T} $, $g_k = g_k + \textbf{c}^d(t)r_{k}(t)$
\STATE \quad\quad$\hat{\mu_k} = B_k^{-1} f$
\STATE \quad\quad$\forall i \in C^d(t)$, $n_i(t)=n_i(t-1)+1$ and $r^f_i(t)=r^f_i(t-1)+1$.
\STATE {\bfseries }\quad\textbf{End if}
 \STATE {\bfseries }\textbf{End do}
 \end{algorithmic}
\end{algorithm}

\end{small}

We now derive an upper bound on the regret of the policy computed by the Thompson Sampling with Restricted Context, or TSRC, algorithm we just presented. We start with introducing some notation: $0 < \epsilon < 1$ represents the parameter of the contextual Thompson Sampling (Algorithm 3), and $\Delta_i=\mu_{C^{d^*}}- \mu_{C^d}$, where $\mu_{C^{d^*}}, \mu_{C^d}$ are the expected rewards of the optimal arm subset $C^{d^*} \in C$ out of all subsets of size $d$, and of the given arm subset $C^d \subseteq C$, $|C^d|=d$, respectively. Our upper bound is based on two key results presented in the following lemmas.

{\small\begin{ex}\label{fact:upperCBTS} \cite{AgrawalG13}
With probability $1-\gamma$, where $0 < \gamma < 1$, the upper bound on the expected regret R(T) for the CTS in the contextual bandit problem with $K$ arms and $d$ features (context size) is given as follows:
\begin{eqnarray*}
E[R(T)]<\frac{d\gamma}{\epsilon} \sqrt{T^{\epsilon+1}} (ln (T) d) ln \frac{1}{\gamma}.
\end{eqnarray*}
\end{ex}}


{\small\begin{ex}\label{fact:uppercom} \cite{KomiyamaHN15}
The upper bound on the regret $R(T)$ for the Thompson Sampling in the bandit problem with the set of $S = \{1,...,K\}$ arms is the following:
\begin{eqnarray*}
E[R(T)]<(\sum_{i\in S}\frac{1}{\Delta_i^2})^2 \ln\ T
\end{eqnarray*}
where $\Delta_i=\mu^*- \mu_i$, where $\mu^*, \mu_i$ are the expected rewards of the optimal arm and of the arm $i \in S$, respectively.
\end{ex}}


Using the results of the above two lemmas, we can derive the following result.
{\small\begin{thm}\label{theorem2}
 With probability $1-\gamma$, where $0 < \gamma < 1$, the expected regret $R(T)$ accumulated by the $TSRC$ algorithm in $T$ iterations is upper-bounded by
\begin{eqnarray*}
E[R(T)]<(\sum_{C^d\in C}\frac{1}{\Delta_{C^d}^2})^2 \ln\ T +\frac{d\gamma}{\epsilon} \sqrt{(T-\tau) ^{\epsilon+1}} (\ln (T-\tau ) d) \ln \frac{1}{\gamma},
\end{eqnarray*}
\end{thm}}
with $\tau < (\sum_{C^d \subseteq C, |C^d|=d}\frac{1}{\Delta_{C^d}^2})^2 ln\ T$.

\begin{proof}
We will split the total regret into two parts,
{\small\begin{eqnarray*}
R(T)=R(\tau_1)+R(\tau_2),
\end{eqnarray*}}
where $\tau_1$ is the number of time points within the first $T$ iterations at which a sub-optimal subset of the features was selected, and $\tau_2 $ is, vice versa, the number of times points when the best subset of the context was used; clearly, $T=\tau_1+\tau_2$.
Note that $	\tau_1= R_{Comb}(T)$, 
where $R_{Comb}(T)$ is the regret of the combinatorial bandit accumulated in the first part of the algorithm when looking for the optimal subset of features. Then
{\small\begin{eqnarray*}
	R(T) = R_{ComB}(T) + R_{CB}(\tau_2),
\end{eqnarray*}}
where $R_{CB}(\tau_2)$ is the regret accumulated by the contextual bandit algorithm, because while the algorithm is playing $\tau_2$ times with the optimal subsets of the context, it is not making mistakes due to the features selection.

Note that the combinatorial bandit setting can be transformed into the standard multi-arm bandit setting, where each subset of arms is treated as a separate arm. Thus, the upper-bound in MAB setting from \cite{KomiyamaHN15}, shown in the Lemma \ref{fact:uppercom}, can be applied in our combinatorial bandit setting, where $\sum_{i \in S}$ will be replaced by $\sum_{C^d \subseteq C, |C^d|=d}$.
Combining this bound with the the result in Lemma \ref{fact:upperCBTS} gives us:
{\small\begin{eqnarray*}
E[R(T)]<(\sum_{M\in S}\frac{1}{\Delta_M^2})^2 \ln\ T
+\frac{d\gamma}{\epsilon} \sqrt{(\tau_2)^{\epsilon+1}} (ln (\tau_2) d) \ln \frac{1}{\gamma},
\end{eqnarray*}}
with $\tau_2 = T- R(T)$, we get our final result.
\end{proof} 

\subsection{Contextual Bandit with Restricted Context in Non-stationary Environment}
%In a stationary environment, we assumed that the distribution of the context vectors, as well as the reward distribution for each arm, are drawn from stationary distributions; the goal of the player is then to find a subset of features allowing for the optimal context-to-arm mapping and stick with this choice. However, the objective changes if the environment becomes non-stationary.
In {\em non-stationary CBRC setting}, we will assume that {\em the rewards distribution can change at certain times, and remain stationary between such changes.} Given the non-stationarity of the reward, the player may need to continue looking for feature subsets which allow for the optimal context-arm mapping, rather than converge to a fixed subset. Similarly to stationary CBRC problem described earlier, at each iteration, a context $c(t)$ describes the environment, and the player has to choose a subset $c^d(t)\in c(t)$ of features from this context to observe; then, based on those observations, the player chooses an arm $k(t)$. The reward $r_{t,k}$ of the played arm is revealed. As we mentioned above, the distribution of the reward is no longer assumed to be stationary; the change-points in distribution of $r_{t,k}$, and the (stationary) distributions of this random variable between the change points are unknown. For now, we will also make a simplifying assumptions that the change points occur at at every $v$ time points, i.e. the windows of stationarity have a fixed size.

We will now derive the lower bound on the expected regret in non-stationary CBRC setting with the above assumptions, for any algorithm solving this problem. The only assumption about the algorithm is that it knows about the fixed-size stationarity windows, but not their actual, size and uses $w$ as an approximation of $v$.
{\small\begin{thm}\label{theorem3}
	Let $v$ be the stationary window size, and let $w$ is the stationary window size set by an algorithm for solving the CBRC problem in a non-stationary environment. Then the accumulated expected regret $R$ is lower-bounded by
	\begin{eqnarray*}
		E[R(T)]> \lfloor T/v \rfloor [\gamma \sqrt{\tau d}+\gamma' \sqrt{(w-\tau)d}],
	\end{eqnarray*}
	with $E(\tau) > m \sqrt{Kw}$.
\end{thm}}
\begin{proof}
	Let us assume that the algorithm's estimate $w$ of the stationary window size is exact, i.e. $w=v$; otherwise, the expected regret would only increase. We can decompose the time window $T$ into ${\lfloor T/v \rfloor }$ stationary intervals, each of length $v=w$, and the remaining interval of length $0 \leq w' < w$. Then the expected regret over $T$ can be lower-bounded by the sum of expected regrets $E(R_s(w))$ for stationary CBRC problem on each stationary window; since there are $\lfloor T/v \rfloor$ such windows, we get
	{\small\begin{eqnarray*}
		E(R(T)) \geq \lfloor T/v \rfloor E(R_s(w)).
	\end{eqnarray*}}
	Combining this bound with the following result of the Theorem \ref{theorem1}
	{\small\begin{eqnarray*}
		E(R_s(w))>\gamma \sqrt{\tau d}+\gamma' \sqrt{(w-\tau)d},
	\end{eqnarray*}}
	where $E(\tau) > m \sqrt{KT}$, concludes the proof.
\end{proof}

\subsubsection{Windows Thompson Sampling with Restricted Context}
\label{subsec:UCB}
Similarly to the TSRC algorithm proposed earlier for the stationary CBRC problem, our algorithm for the non-stationary CBRC uses Thompson Sampling (TS) to find the best $d$ features of the context. The two algorithms are practically identical, except for the following important detail: instead of updating the Beta distribution with the number of successes and failures accumulated from the beginning of the game, we will now count only the successes and failures within a given stationarity window introduced in the previous section. The resulting approach is called the {\em Window Thompson Sampling with restricted Context}, or {\em WTSRC}.

We will now derive the upper bound on the expected regret of the WTSRC
algorithm; we no longer assume the perfect knowledge of $v$, the actual size of the stationarity window, and consider the two cases, $v \leq w$ and $v > w$, where $w$ is the stationarity window size estimate used by the algorithm.

{\small\begin{thm}\label{theorem4}
	Let $v$ be the stationary window size, and let $w$ is the stationary window size set by the $WTSRC$ algorithm for solving the CBRC problem in a non-stationary environment. Then, with probability $1-\gamma$, where $0 < \gamma < 1$, the expected regret $R(T)$ accumulated in $T$ iterations by the algorithm can be upper-bounded as follows:
{\small	\begin{eqnarray*}
		E[R(T)] \leq \lceil T/w \rceil ( R^U(x)+w-x), ~0 \leq x \leq v
	\end{eqnarray*}}
	when $v \leq w$, and
{\small	\begin{eqnarray*}
		E[R(T)] \leq \lceil T/w \rceil (\lfloor v/w \rfloor R(w) + w),
	\end{eqnarray*}}
	when $v > w$, where $R^{U}(t)$ denotes the upper bound on the expected regret of the TSRC algorithm in the stationary CBRC problem over $t$ iterations, given by the Theorem \ref{theorem2}:
	{\small\begin{eqnarray*}
		R^U(t)=(\sum_{M\in S}\frac{1}{\Delta_M^2})^2 \ln\ t +\frac{d\gamma}{\epsilon} \sqrt{(T-\tau) ^{\epsilon+1}} (\ln (t-\tau ) d) \ln \frac{1}{\gamma},
	\end{eqnarray*}}
	with $\tau < (\sum_{M\in S}\frac{1}{\Delta_M^2})^2 \ln\ t$.
\end{thm}}
\begin{proof}	
	We consider first the case when the size of the stationarity window does not exceed the window size assumed by the algorithm, i.e. $v \leq w$. Within $T$ iterations, the $WTSRC$ algorithm goes through at most $\lceil T/w \rceil$ cycles, each of length $w$, where the algorithm assumes a stationary input at each cycle. Let $ 0 \leq x \leq v$ denote the first change point within a cycle of length $w$, i.e. the point at which the input distribution changes. Then, the expected regret for this cycle can be bounded by $R^U(x) + w-x$, since, until the change point, the regret is accumulated in the same way as in TSRC algorithm for stationary environment as for the stationary environment, and after the change point, until the end of the algorithm's cycle of length $w$, the algorithm will make at most $w-x$ mistakes. Then, over $T$ iterations, the total expected regret can be upper-bounded by
	{\small\begin{eqnarray*}
		E(R(T)) \leq \lceil T/w \rceil (R^U(x)+w-x),
	\end{eqnarray*}}
	which concludes the first part of the proof.
	Next, we consider the case when $v > w$, i.e. when the actual window of stationarity size exceeds the algorithm's stationarity window size. There are at most $\lceil T/v \rceil$ (actual) windows of stationarity within the $T$ iterations; within each such window of size $v$, there are $\lfloor v/w \rfloor $ cycles of the algorithm which {\em start} within the true stationarity window, each accumulating expected reward $R(w)$;
	the remaining number of time points $v - w \lfloor v/w \rfloor \leq w$,
	may belong to an algorithmic cycle (of length $w$) which started outside of the current stationary window, and thus the algorithm might be making mistakes at all those time points, in the worst case, thus yielding the upper bound on the expected regret
{\small\begin{eqnarray*}
		E[R(T)] \leq \lceil T/w \rceil (\lfloor v/w \rfloor R(w) + w).
	\end{eqnarray*}}
	which concludes the second part of the proof for the case of $v > w$.
\end{proof} 

==> theory_nonstationary.tex <==
We will now derive the upper bound on the expected regret of the WTSRC
algorithm; we no longer assume the perfect knowledge of $v$, the actual size of the stationarity window, and consider the two cases, $v \leq w$ and $v > w$, where $w$ is the stationarity window size   assumed  by the algorithm $WTSRC$ and specified as an input parameter.

{\small\begin{thm}\label{theorem4}
Let $v$ be the stationary window size, and let $w$ is the stationary window size set by the $WTSRC$ algorithm for solving the CBRC problem with linear payoff in a non-stationary environment. Then, with probability $1-\gamma$, where $0 < \gamma < 1$, the expected regret $R(T)$ accumulated in $T$ iterations by the algorithm can be upper-bounded as follows:
{\small	\begin{eqnarray*}
		E[R(T)] \leq \lceil T/w \rceil ( R^U(x)+w-x), ~0 \leq x \leq v
	\end{eqnarray*}}
	when $v \leq w$, and
{\small	\begin{eqnarray*}
		E[R(T)] \leq \lceil T/w \rceil (\lfloor v/w \rfloor R(w) + w),
	\end{eqnarray*}}
	when $v > w$, where $R^{U}(t)$ denotes the upper bound on the expected regret of the TSRC algorithm in the stationary CBRC problem over $t$ iterations, given by the Theorem \ref{theorem2}:
	{\small\begin{eqnarray*}
		R^U(t)=(\sum_{C^d \subseteq C, |C^d| = d}\frac{1}{\Delta_{C^d}^2})^2 \ln\ t +\frac{d\gamma}{\epsilon} \sqrt{(T-\tau) ^{\epsilon+1}} (\ln (t-\tau ) d) \ln \frac{1}{\gamma},
	\end{eqnarray*}}
	with $E[\tau] < (\sum_{C^d \subseteq C, |C^d| = d}\frac{1}{\Delta_{C^d}^2})^2 \ln\ t$.
\end{thm}}
\begin{proof}	
	We consider first the case when the size of the stationarity window does not exceed the window size assumed by the algorithm, i.e. $v \leq w$. Within $T$ iterations, the $WTSRC$ algorithm goes through at most $\lceil T/w \rceil$ cycles, each of length $w$, where the algorithm assumes a stationary input at each cycle. Let $ 0 \leq x \leq v$ denote the first change point within a cycle of length $w$, i.e. the point at which the input distribution changes. Then, the expected regret for this cycle can be bounded by $R^U(x) + w-x$, since, until the change point, the regret is accumulated in the same way as in TSRC algorithm for stationary environment as for the stationary environment, and after the change point, until the end of the algorithm's cycle of length $w$, the algorithm will make at most $w-x$ mistakes. Then, over $T$ iterations, the total expected regret can be upper-bounded by
	{\small\begin{eqnarray*}
		E(R(T)) \leq \lceil T/w \rceil (R^U(x)+w-x),
	\end{eqnarray*}}
	which concludes the first part of the proof.
	Next, we consider the case when $v > w$, i.e. when the actual window of stationarity size exceeds the algorithm's stationarity window size. There are at most $\lceil T/v \rceil$ (actual) windows of stationarity within the $T$ iterations; within each such window of size $v$, there are $\lfloor v/w \rfloor $ cycles of the algorithm which {\em start} within the true stationarity window, each accumulating expected reward $R(w)$;
	the remaining number of time points $v - w \lfloor v/w \rfloor \leq w$,
	may belong to an algorithmic cycle (of length $w$) which started outside of the current stationary window, and thus the algorithm might be making mistakes at all those time points, in the worst case, thus yielding the upper bound on the expected regret
{\small\begin{eqnarray*}
		E[R(T)] \leq \lceil T/w \rceil (\lfloor v/w \rfloor R(w) + w).
	\end{eqnarray*}}
	which concludes the second part of the proof for the case of $v > w$.
\end{proof} 

==> theory_stationary.tex <==
We now derive an upper bound on the regret of the policy computed by the Thompson Sampling with Restricted Context, or TSRC, algorithm we just presented. We start with introducing some notation: $0 < \epsilon < 1$ represents the parameter of the contextual Thompson Sampling, %(Algorithm 3),
and $\Delta_{C^d}=\mu_{C^{d^*}}- \mu_{C^d}$, where $\mu_{C^{d^*}}, \mu_{C^d}$ are the expected rewards of the optimal arm subset $C^{d^*} \in C$ out of all subsets of size $d$, and of the given arm subset $C^d \subseteq C$, respectively. Our upper bound is based on two key results presented in the following lemmas.

{\small\begin{ex}\label{fact:upperCBTS} \cite{AgrawalG13}
With probability $1-\gamma$, where $0 < \gamma < 1$, the upper bound on the expected regret R(T) for the Contextual Thompson Sampling algorithm in the CMAB with linear payoff with $K$ arms and $d$ features (context size) is given as follows:
\begin{eqnarray*}
E[R(T)]<\frac{d\gamma}{\epsilon} \sqrt{T^{\epsilon+1}} (ln (T) d) ln \frac{1}{\gamma}.
\end{eqnarray*}
\end{ex}}


{\small\begin{ex}\label{fact:uppercom} \cite{KomiyamaHN15}
The upper bound on the regret $R(T)$ for the Thompson Sampling in the bandit problem with the set of $S = \{1,...,K\}$ arms is the following:
\begin{eqnarray*}
E[R(T)]<(\sum_{i\in S}\frac{1}{\Delta_i^2})^2 \ln\ T
\end{eqnarray*}
where $\Delta_i=\mu^*- \mu_i$, where $\mu^*, \mu_i$ are the expected rewards of the optimal arm and of the arm $i \in S$, respectively.
\end{ex}}

Using the results of the above two lemmas, we can derive the following result.
{\small\begin{thm}\label{theorem2}
In the CMAB with linear payoff, with probability $1-\gamma$, where $0 < \gamma < 1$, the expected regret $R(T)$ accumulated by the $TSRC$ algorithm in $T$ iterations is upper-bounded as follows:
\begin{eqnarray*} E[R(T)]<(\sum_{C^d\in C}\frac{1}{\Delta_{C^d}^2})^2 \ln\ T + \\
+\frac{d\gamma}{\epsilon} \sqrt{(T-\tau) ^{\epsilon+1}} (\ln (T-\tau ) d) \ln \frac{1}{\gamma},
\end{eqnarray*}
\end{thm}}
with $E[\tau] < (\sum_{C^d \subseteq C}\frac{1}{\Delta_{C^d}^2})^2 ln\ T$.

\begin{proof}
We will split the total regret into two parts,
{\small\begin{eqnarray*}
R(T)=R(\tau_1)+R(\tau_2),
\end{eqnarray*}}
where $\tau_1$ is the number of time points within the first $T$ iterations at which a sub-optimal subset of the features was selected, and $\tau_2 $ is, vice versa, the number of times points when the best subset of the context was used; clearly, $T=\tau_1+\tau_2$.
Note that $	\tau_1= R_{Comb}(T)$,
where $R_{Comb}(T)$ is the regret of the combinatorial bandit accumulated in the first part of the algorithm when looking for the optimal subset of features. Then
{\small\begin{eqnarray*}
	R(T) = R_{ComB}(T) + R_{CB}(\tau_2),
\end{eqnarray*}}
where $R_{CB}(\tau_2)$ is the regret accumulated by the contextual bandit algorithm, because while the algorithm is playing $\tau_2$ times with the optimal subsets of the context, it is not making mistakes due to the features selection.

Note that the combinatorial bandit setting can be transformed into the standard multi-arm bandit setting, where each subset of arms is treated as a separate arm. Thus, the upper-bound in MAB setting from \cite{KomiyamaHN15}, shown in the Lemma \ref{fact:uppercom}, can be applied in our combinatorial bandit setting, where $\sum_{i \in S}$ will be replaced by $\sum_{C^d \subseteq C}$.
Combining this bound with the the result in Lemma \ref{fact:upperCBTS} gives us:
{\small\begin{eqnarray*}
E[R(T)]<(\sum_{C^d \subseteq C}\frac{1}{\Delta_{C^d}^2})^2 \ln\ T
+\frac{d\gamma}{\epsilon} \sqrt{(\tau_2)^{\epsilon+1}} (ln (\tau_2) d) \ln \frac{1}{\gamma},
\end{eqnarray*}}
with $\tau_2 = T - R(T)$, we get our final result.
\end{proof}

